Deep learning observables in computational fluid dynamics

Many large scale problems in computational fluid dynamics such as uncertainty quantification, Bayesian inversion, data assimilation and PDE constrained optimization are considered very challenging computationally as they require a large number of expensive (forward) numerical solutions of the corresponding PDEs. We propose a machine learning algorithm, based on deep artificial neural networks, that predicts the underlying \emph{input parameters to observable} map from a few training samples (computed realizations of this map). By a judicious combination of theoretical arguments and empirical observations, we find suitable network architectures and training hyperparameters that result in robust and efficient neural network approximations of the parameters to observable map. Numerical experiments are presented to demonstrate low prediction errors for the trained network networks, even when the network has been trained with a few samples, at a computational cost which is several orders of magnitude lower than the underlying PDE solver. Moreover, we combine the proposed deep learning algorithm with Monte Carlo (MC) and Quasi-Monte Carlo (QMC) methods to efficiently compute uncertainty propagation for nonlinear PDEs. Under the assumption that the underlying neural networks generalize well, we prove that the deep learning MC and QMC algorithms are guaranteed to be faster than the baseline (quasi-) Monte Carlo methods. Numerical experiments demonstrating one to two orders of magnitude speed up over baseline QMC and MC algorithms, for the intricate problem of computing probability distributions of the observable, are also presented.

==> added.tex <==
\section{NEW LAX SOD PLOTS}
All domains are $[-5, 5]$, we set the end time $T=1.5$, used $3000$ samples.
\section{The Sod Shock Tube}
\subsection{Problem description}

1D Euler, $\gamma=1.4$, two states: 
We let the left state be given as
\begin{align*}
\rho_L&\sim \U[0.3, 1.2]\\
w_L&\sim \U[0, 1]\\
p_L&\sim\U[0.9, 4.1]
\end{align*}
and the right state
\begin{align*}
\rho_R&\sim \U[0.1, 0.7]\\
w_R&=0\\
p_R&\sim \U[0.05, 0.7].
\end{align*}
The shock location is given as $X\sim \U[-0.5, 0.5]$. 

Training data on 128 QMC points. mesh resolution 2048. Total validation samples: 16256



\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/rho_mean_std_0}
	
	\caption{$\rho$ at $t=0$.}
\end{figure}

\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/rho_mean_std_1}
	
	\caption{$\rho$ at $t=1.5$.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/mx_mean_std_0}
	
	\caption{$m_x$ at $t=0$.}
\end{figure}

\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/mx_mean_std_1}
	
	\caption{$m_x$ at $t=1.5$.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/E_mean_std_0}
	
	\caption{$E$ at $t=0$.}
\end{figure}

\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/E_mean_std_1}
	
	\caption{$E$ at $t=1.5$.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/p_mean_std_0}
	
	\caption{$p$ at $t=0$.}
\end{figure}

\begin{figure}
	\includegraphics[width=0.8\textwidth]{img/p_mean_std_1}
	
	\caption{$p$ at $t=1.5$.}
\end{figure}




\begin{figure}
	\subfigure[$Q_1$]{\includegraphics[width=0.5\textwidth]{img/laxsodhist_prediction_l2_relative_q1_allconfigurationsbestperforming_128_ordinary_notitle.png}}
	\subfigure[$Q_2$]{\includegraphics[width=0.5\textwidth]{img/laxsodhist_prediction_l2_relative_q2_allconfigurationsbestperforming_128_ordinary_notitle.png}}
	\subfigure[$Q_3$]{\includegraphics[width=0.5\textwidth]{img/laxsodhist_prediction_l2_relative_q3_allconfigurationsbestperforming_128_ordinary_notitle.png}}
	\caption{lax sod histogram all configurations.}

\end{figure}

\begin{figure}
	\subfigure[$Q_1$]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_sgd_adam_128_ordinary_bestperforming_notitle.png}} 
	\subfigure[$Q_2$]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_sgd_adam_128_ordinary_bestperforming_notitle.png}} 
	\subfigure[$Q_3$]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_sgd_adam_128_ordinary_bestperforming_notitle.png}} 
	\caption{Histograms for the relative prediction errors comparing the ADAM and SGD algorithms on the lax sod shock tube}
	
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure}
	\subfigure[Q1]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_goodadam_badadam_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q2]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_goodadam_badadam_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q3]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_goodadam_badadam_128_ordinary_bestperforming_notitle.png}}
	\caption{Histograms of the relative prediction errors, comparing \emph{Good} ADAM and \emph{bad} ADAM, for the LAX SOD.}

\end{figure}

\begin{figure}
	\subfigure[Q1]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_goodadammse_goodadammae_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q2]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_goodadammse_goodadammae_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q3]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_goodadammse_goodadammae_128_ordinary_bestperforming_notitle.png}}
	\caption{Histograms for the relative prediction errors, comparing the mean absolute error and mean square error loss functions, for theLAX SOD}

\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}
	\subfigure[Q1]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_goodadaml1reg_goodadaml2reg_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q2]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_goodadaml1reg_goodadaml2reg_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q3]{\includegraphics[width=0.48\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_goodadaml1reg_goodadaml2reg_128_ordinary_bestperforming_notitle.png}}
	\caption{Histograms for the relative prediction error, comparing $L^1$ and $L^2$ regularizations of the loss function, for the LAX SOD}
	\label{fig:afoilreg}
\end{figure}

\begin{figure}
	\subfigure[Q1]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_goodadamwithval_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}} 
	\subfigure[Q1]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_goodadamwithtrain_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q1]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q1_goodadamwithmeantrain_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q2]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_goodadamwithval_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}} 
	\subfigure[Q2]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_goodadamwithtrain_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q2]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q2_goodadamwithmeantrain_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q3]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_goodadamwithval_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}} 
	\subfigure[Q3]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_goodadamwithtrain_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}}
	\subfigure[Q3]{\includegraphics[width=0.32\textwidth]{img/laxsodcomparison_histogram_prediction_l2_relative_q3_goodadamwithmeantrain_goodadamwithwasstrain_128_ordinary_bestperforming_notitle.png}}
	\caption{LAX SODNetwork performance with respect to selection criteria for retrainings (see section \ref{sec:imp} i.e, \emph{train,val,mean-train,wass-train} for the flow past airfoils problem. We compare \emph{wass-train} with each of the other three criteria. Histograms for prediction error (X-axis) with number of configurations (Y-axis) are shown.}

\end{figure}


\begin{figure}
\subfigure[Q1]{\includegraphics[width=0.48\textwidth]{img/laxsodtraining_size_prediction_l2_relative_q1_ordinary_onlyadamwithl2andlowregularizationorl1withregularizationbestperforming_sel_min_max_notitle.png}} 
\subfigure[Q2]{\includegraphics[width=0.48\textwidth]{img/laxsodtraining_size_prediction_l2_relative_q2_ordinary_onlyadamwithl2andlowregularizationorl1withregularizationbestperforming_sel_min_max_notitle.png}} 
\subfigure[Q3]{\includegraphics[width=0.48\textwidth]{img/laxsodtraining_size_prediction_l2_relative_q3_ordinary_onlyadamwithl2andlowregularizationorl1withregularizationbestperforming_sel_min_max_notitle.png}} 
\caption{LAX SOD Relative percentage mean square prediction error \eqref{eq:perr} (Y-axis) for the neural networks approximating the flow past airfoils problem, with respect to number of training samples (X-axis). For each number of training samples, we plot the mean, minimum and maximum (over hyperparameter configurations) of the prediction error. Only the selected (optimal) retraining is shown. }

\end{figure}




\begin{figure}
	\subfigure[Q1]{\includegraphics[width=0.5\textwidth]{img/laxsodtraining_size_wasserstein_speedup_real_q1_ordinary_allconfigurationsbestperforming_sel_max_notitle.png}} 
	\subfigure[Q2]{\includegraphics[width=0.5\textwidth]{img/laxsodtraining_size_wasserstein_speedup_real_q2_ordinary_allconfigurationsbestperforming_sel_max_notitle.png}} 
	\subfigure[Q3]{\includegraphics[width=0.5\textwidth]{img/laxsodtraining_size_wasserstein_speedup_real_q3_ordinary_allconfigurationsbestperforming_sel_max_notitle.png}} 
	\caption{LAX SOD Real speedups \eqref{eq:esp1} for the DLQMC algorithm over the baseline QMC algorithm (Y-axis) with respect to number of training samples (X-axis) for the flows past airfoils problem. The maximum and mean speed up (over all hyperparameter configurations)  are shown.}

\end{figure}

